Plastically-driven variation of elastic stiffness in green bodies during powder compaction: Part I Experiments and elastoplastic coupling

Cold compaction of ceramic powders is driven by plastic strain, during which the elastic stiffness of the material progressively increases from values typical of granular matter to those representative of a fully dense solid. This increase of stiffness strongly affects the mechanical behaviour of the green body and is crucial in the modelling of forming processes for ceramics. A protocol for ultrasonic experimental investigation (via P and S waves transmission) is proposed to quantify the elastic constants (Young modulus and Poisson's ratio) as functions of the forming pressure. Experimental results performed in uniaxial strain allow for the introduction of laws that describe the variation of the elastic constants during densification. These laws are motivated in terms of elastoplastic coupling through the simulation of an isostatic pressure compaction process of alumina powder. A micromechanical explanation of the stiffening of elastic properties during densification is deferred to Part II of this study.

==> definitions.tex <==
%Definitions: general
\newcommand{\singlespace}{\baselineskip=12pt \lineskiplimit=0pt \lineskip=0pt}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\lb}{\label}
\newcommand{\beqar}{\begin{eqnarray}}
\newcommand{\eeqar}{\end{eqnarray}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\benum}{\begin{enumerate}}
\newcommand{\eenum}{\end{enumerate}}
\newcommand{\barr}{\begin{array}}
\newcommand{\earr}{\end{array}}
\def\ds{\displaystyle}
\newcommand\eq[1]{(\ref{#1})}
\newcommand{\bfm}[1]{\mbox{\boldmath ${#1}$}}        % produces bold math symbol

%Definitions: theorem
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{remark}{Remark}[section]
% \newtheorem{corollary}{Corollary}[section]

%Definitions: symbols
% \newcommand{\jump}[2]{[\mbox{\hspace{-#1em}}[#2]\mbox{\hspace{-#1em}}]}
% dopodiche' scrivi il comando
% \jump{*}{**}
% dove * e' un numero mentre ** e' quello che tu vuoi tra parentesi.
% Il numero serve a far si che le due parentesi quadre che comporranno
% l'unica parentesi che tu vuoi siano ben posizionate. Tale numero varia a
% seconda di chi sia **.

% \newcommand{\bjump}[2]{\left[\mbox{\hspace{-#1em}}\left[#2\right]\mbox{\hspace{-#1em}}\right]}
% con parentesi di altezza variabile

\def\scalp{\mbox{\boldmath $\, \cdot \,$}}
\def\bob{{\, \underline{\overline{\otimes}} \,}}
%\def\bob{\makebox{\raisebox{-.215ex}{$\Box$}\hspace{-.73em}$\scalp$}}
\def\gdp{\ \begin{picture}
           (6,6)\put(0,0){\framebox(6,6){$\times$}}
           \end{picture} \ }
%\def\gdp{\makebox{\raisebox{-.215ex}{$\Box$}\hspace{-.778em}$\times$}}
\def\sop{{\, \overline{\otimes} \,}}
\def\sot{{\, \underline{\otimes} \,}}
\newcommand{\deriv}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\nderiv}[3]{\frac{\partial^{\,#3} #1}{\partial #2^{\,#3}}}
\newcommand{\maxx}[2]{\text{Max}_{#1}\ \left(#2\right)}
\newcommand{\oldr}[1]{\stackrel{\circ}{\mbox{#1}}}
%\newcommand{\pv}{-\mskip-19mu\int}
\newcommand{\modI}{\text{I}}
\newcommand{\modII}{\text{II}}
\newcommand{\modIII}{\text{III}}
\def\Xint#1{\mathchoice
   {\XXint\displaystyle\textstyle{#1}}%
   {\XXint\textstyle\scriptstyle{#1}}%
   {\XXint\scriptstyle\scriptscriptstyle{#1}}%
   {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
   \!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}
   \vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
\def\fp{\Xint=}
\def\pv{\Xint-}

%Definitions: vectors and points and second-order tensor
\def\b0{\mbox{\boldmath $0$}}
\def\ba{\mbox{\boldmath $a$}}
\def\bb{\mbox{\boldmath $b$}}
\def\bc{\mbox{\boldmath $c$}}
\def\bd{\mbox{\boldmath $d$}}
\def\be{\mbox{\boldmath $e$}}
\def\beffe{\mbox{\boldmath $f$}}
\def\bg{\mbox{\boldmath $g$}}
\def\bh{\mbox{\boldmath $h$}}
\def\bi{\mbox{\boldmath $i$}}
\def\bj{\mbox{\boldmath $j$}}
\def\bk{\mbox{\boldmath $k$}}
\def\bl{\mbox{\boldmath $l$}}
\def\bm{\mbox{\boldmath $m$}}
\def\bn{\mbox{\boldmath $n$}}
\def\bo{\mbox{\boldmath $o$}}
\def\bp{\mbox{\boldmath $p$}}
\def\bq{\mbox{\boldmath $q$}}
\def\br{\mbox{\boldmath $r$}}
\def\bs{\mbox{\boldmath $s$}}
\def\bt{\mbox{\boldmath $t$}}
\def\bu{\mbox{\boldmath $u$}}
\def\bv{\mbox{\boldmath $v$}}
\def\bw{\mbox{\boldmath $w$}}
\def\bx{\mbox{\boldmath $x$}}
\def\by{\mbox{\boldmath $y$}}
\def\bz{\mbox{\boldmath $z$}}
\def\bA{\mbox{\boldmath $A$}}
\def\bB{\mbox{\boldmath $B$}}
\def\bC{\mbox{\boldmath $C$}}
\def\bD{\mbox{\boldmath $D$}}
\def\bE{\mbox{\boldmath $E$}}
\def\bF{\mbox{\boldmath $F$}}
\def\bG{\mbox{\boldmath $G$}}
\def\bH{\mbox{\boldmath $H$}}
\def\bI{\mbox{\boldmath $I$}}
\def\bJ{\mbox{\boldmath $J$}}
\def\bK{\mbox{\boldmath $K$}}
\def\bL{\mbox{\boldmath $L$}}
\def\bM{\mbox{\boldmath $M$}}
\def\bN{\mbox{\boldmath $N$}}
\def\bO{\mbox{\boldmath $O$}}
\def\bP{\mbox{\boldmath $P$}}
\def\bQ{\mbox{\boldmath $Q$}}
\def\bR{\mbox{\boldmath $R$}}
\def\bS{\mbox{\boldmath $S$}}
\def\bT{\mbox{\boldmath $T$}}
\def\bU{\mbox{\boldmath $U$}}
\def\bV{\mbox{\boldmath $V$}}
\def\bW{\mbox{\boldmath $W$}}
\def\bX{\mbox{\boldmath $X$}}
\def\bY{\mbox{\boldmath $Y$}}
\def\bZ{\mbox{\boldmath $Z$}}

\def\Id{\mbox{\boldmath $I$}}
\newcommand{\bsigma}{\mbox{\boldmath $\sigma$}}
\newcommand{\bSigma}{\mbox{\boldmath $\Sigma$}}
\newcommand{\bepsilon}{\mbox{\boldmath $\epsilon$}}
\newcommand{\bvarepsilon}{\mbox{\boldmath $\varepsilon$}}
\newcommand{\btau}{\mbox{\boldmath $\tau$}}
\newcommand{\bpsi}{\mbox{\boldmath$\psi$}}
\newcommand{\bPsi}{\mbox{\boldmath$\Psi$}}
\newcommand{\bxi}{\mbox{\boldmath $\xi$}}
\newcommand{\bphi}{\mbox{\boldmath $\phi$}}
\newcommand{\bvarphi}{\mbox{\boldmath$\varphi$}}
\newcommand{\bPhi}{\mbox{\boldmath $\Phi$}}
\newcommand{\bXi}{\mbox{\boldmath $\Xi$}}
\newcommand{\bchi}{\mbox{\boldmath $\chi$}}
\newcommand{\bmu}{\mbox{\boldmath $\mu$}}

%Definitions: fourth-order tensors
\def\f0{\ensuremath{\mathbb{O}}}
\def\fA{\ensuremath{\mathbb{A}}}
\def\fB{\ensuremath{\mathbb{B}}}
\def\fC{\ensuremath{\mathbb{C}}}
\def\fD{\ensuremath{\mathbb{D}}}
\def\fE{\ensuremath{\mathbb{E}}}
\def\fF{\ensuremath{\mathbb{F}}}
\def\fG{\ensuremath{\mathbb{G}}}
\def\fH{\ensuremath{\mathbb{H}}}
\def\fI{\ensuremath{\mathbb{I}}}
\def\fJ{\ensuremath{\mathbb{J}}}
\def\fK{\ensuremath{\mathbb{K}}}
\def\fL{\ensuremath{\mathbb{L}}}
\def\fM{\ensuremath{\mathbb{M}}}
\def\fN{\ensuremath{\mathbb{N}}}
\def\fO{\ensuremath{\mathbb{O}}}
\def\fP{\ensuremath{\mathbb{P}}}
\def\fQ{\ensuremath{\mathbb{Q}}}
\def\fR{\ensuremath{\mathbb{R}}}
\def\fS{\ensuremath{\mathbb{S}}}
\def\fT{\ensuremath{\mathbb{T}}}
\def\fU{\ensuremath{\mathbb{U}}}
\def\fV{\ensuremath{\mathbb{V}}}
\def\fW{\ensuremath{\mathbb{W}}}
\def\fX{\ensuremath{\mathbb{X}}}
\def\fY{\ensuremath{\mathbb{Y}}}
\def\fZ{\ensuremath{\mathbb{Z}}}

% Abbreviate definitions of greek symbols
\newcommand{\Ga}{\alpha}
\newcommand{\Gb}{\beta}
\newcommand{\Gd}{\delta}
\newcommand{\Ge}{\epsilon}
\newcommand{\Gve}{\varepsilon}
\newcommand{\Gf}{\phi}
\newcommand{\Gvf}{\varphi}
\newcommand{\Gg}{\gamma}
\newcommand{\Gc}{\chi}
\newcommand{\Gi}{\iota}
\newcommand{\Gk}{\kappa}
\newcommand{\Gl}{\lambda}
\newcommand{\Gn}{\eta}
\newcommand{\Gm}{\mu}
\newcommand{\Gv}{\nu}
\newcommand{\Gp}{\pi}
\newcommand{\Gt}{\theta}
\newcommand{\Gvt}{\vartheta}
\newcommand{\Gr}{\rho}
\newcommand{\Gvr}{\varrho}
\newcommand{\Gs}{\sigma}
\newcommand{\Gvs}{\varsigma}
\newcommand{\Gj}{\tau}
\newcommand{\Gu}{\upsilon}
\newcommand{\Go}{\omega}
\newcommand{\Gx}{\xi}
\newcommand{\Gy}{\psi}
\newcommand{\Gz}{\zeta}
\newcommand{\GD}{\Delta}
\newcommand{\GF}{\Phi}
\newcommand{\GG}{\Gamma}
\newcommand{\GL}{\Lambda}
\newcommand{\GP}{\Pi}
\newcommand{\GT}{\Theta}
\newcommand{\GS}{\Sigma}
\newcommand{\GU}{\Upsilon}
\newcommand{\GO}{\Omega}
\newcommand{\GX}{\Xi}
\newcommand{\GY}{\Psi}

% Abbreviate definitions of bold greek symbols
\newcommand{\BGa}{\bfm\alpha}
\newcommand{\BGb}{\bfm\beta}
\newcommand{\BGd}{\bfm\delta}
\newcommand{\BGe}{\bfm\epsilon}
\newcommand{\BGve}{\bfm\varepsilon}
\newcommand{\BGf}{\bfm\phi}
\newcommand{\BGvf}{\bfm\varphi}
\newcommand{\BGg}{\bfm\gamma}
\newcommand{\BGc}{\bfm\chi}
\newcommand{\BGi}{\bfm\iota}
\newcommand{\BGk}{\bfm\kappa}
\newcommand{\BGl}{\bfm\lambda}
\newcommand{\BGn}{\bfm\eta}
\newcommand{\BGm}{\bfm\mu}
\newcommand{\BGv}{\bfm\nu}
\newcommand{\BGp}{\bfm\pi}
\newcommand{\BGt}{\bfm\theta}
\newcommand{\BGvt}{\bfm\vartheta}
\newcommand{\BGr}{\bfm\rho}
\newcommand{\BGvr}{\bfm\varrho}
\newcommand{\BGs}{\bfm\sigma}
\newcommand{\BGvs}{\bfm\varsigma}
\newcommand{\BGj}{\bfm\tau}
\newcommand{\BGu}{\bfm\upsilon}
\newcommand{\BGo}{\bfm\omega}
\newcommand{\BGx}{\bfm\xi}
\newcommand{\BMx}{\bfm\xi}
\newcommand{\BGy}{\bfm\psi}
\newcommand{\BGz}{\bfm\zeta}
\newcommand{\BGD}{\bfm\Delta}
\newcommand{\BGF}{\bfm\Phi}
\newcommand{\BGG}{\bfm\Gamma}
\newcommand{\BGL}{\bfm\Lambda}
\newcommand{\BGP}{\bfm\Pi}
\newcommand{\BGT}{\bfm\Theta}
\newcommand{\BGS}{\bfm\Sigma}
\newcommand{\BGU}{\bfm\Upsilon}
\newcommand{\BGO}{\bfm\Omega}
\newcommand{\BGX}{\bfm\Xi}
\newcommand{\BGY}{\bfm\Psi}

%Definitions: calligraphic letters
\newcommand{\mA}{\ensuremath{\mathcal{A}}}
\newcommand{\mB}{\ensuremath{\mathcal{B}}}
\newcommand{\mC}{\ensuremath{\mathcal{C}}}
\newcommand{\mD}{\ensuremath{\mathcal{D}}}
\newcommand{\mE}{\ensuremath{\mathcal{E}}}
\newcommand{\mF}{\ensuremath{\mathcal{F}}}
\newcommand{\mG}{\ensuremath{\mathcal{G}}}
\newcommand{\mH}{\ensuremath{\mathcal{H}}}
\newcommand{\mI}{\ensuremath{\mathcal{I}}}
\newcommand{\mJ}{\ensuremath{\mathcal{J}}}
\newcommand{\mK}{\ensuremath{\mathcal{K}}}
\newcommand{\mL}{\ensuremath{\mathcal{L}}}
\newcommand{\mM}{\ensuremath{\mathcal{M}}}
\newcommand{\mN}{\ensuremath{\mathcal{N}}}
\newcommand{\mO}{\ensuremath{\mathcal{O}}}
\newcommand{\mP}{\ensuremath{\mathcal{P}}}
\newcommand{\mQ}{\ensuremath{\mathcal{Q}}}
\newcommand{\mR}{\ensuremath{\mathcal{R}}}
\newcommand{\mS}{\ensuremath{\mathcal{S}}}
\newcommand{\mT}{\ensuremath{\mathcal{T}}}
\newcommand{\mU}{\ensuremath{\mathcal{U}}}
\newcommand{\mV}{\ensuremath{\mathcal{V}}}
\newcommand{\mW}{\ensuremath{\mathcal{W}}}
\newcommand{\mX}{\ensuremath{\mathcal{X}}}
\newcommand{\mY}{\ensuremath{\mathcal{Y}}}
\newcommand{\mZ}{\ensuremath{\mathcal{Z}}}

%Definitions: bold calligraphic letters
\newcommand{\bmA}{\mbox{\boldmath $\mathcal{A}$}}
\newcommand{\bmB}{\mbox{\boldmath $\mathcal{B}$}}
\newcommand{\bmC}{\mbox{\boldmath $\mathcal{C}$}}
\newcommand{\bmD}{\mbox{\boldmath $\mathcal{D}$}}
\newcommand{\bmE}{\mbox{\boldmath $\mathcal{E}$}}
\newcommand{\bmF}{\mbox{\boldmath $\mathcal{F}$}}
\newcommand{\bmG}{\mbox{\boldmath $\mathcal{G}$}}
\newcommand{\bmH}{\mbox{\boldmath $\mathcal{H}$}}
\newcommand{\bmI}{\mbox{\boldmath $\mathcal{I}$}}
\newcommand{\bmJ}{\mbox{\boldmath $\mathcal{J}$}}
\newcommand{\bmK}{\mbox{\boldmath $\mathcal{K}$}}
\newcommand{\bmL}{\mbox{\boldmath $\mathcal{L}$}}
\newcommand{\bmM}{\mbox{\boldmath $\mathcal{M}$}}
\newcommand{\bmN}{\mbox{\boldmath $\mathcal{N}$}}
\newcommand{\bmO}{\mbox{\boldmath $\mathcal{O}$}}
\newcommand{\bmP}{\mbox{\boldmath $\mathcal{P}$}}
\newcommand{\bmQ}{\mbox{\boldmath $\mathcal{Q}$}}
\newcommand{\bmR}{\mbox{\boldmath $\mathcal{R}$}}
\newcommand{\bmS}{\mbox{\boldmath $\mathcal{S}$}}
\newcommand{\bmT}{\mbox{\boldmath $\mathcal{T}$}}
\newcommand{\bmU}{\mbox{\boldmath $\mathcal{U}$}}
\newcommand{\bmV}{\mbox{\boldmath $\mathcal{V}$}}
\newcommand{\bmW}{\mbox{\boldmath $\mathcal{W}$}}
\newcommand{\bmX}{\mbox{\boldmath $\mathcal{X}$}}
\newcommand{\bmY}{\mbox{\boldmath $\mathcal{Y}$}}
\newcommand{\bmZ}{\mbox{\boldmath $\mathcal{Z}$}}

%Definitions: functions
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\dev}{\mathop{\mathrm{dev}}}
\newcommand{\diver}{\mathop{\mathrm{div}}}
\newcommand{\Div}{\mathop{\mathrm{Div}}}
\newcommand{\grad}{\mathop{\mathrm{grad}}}
\newcommand{\Grad}{\mathop{\mathrm{Grad}}}
\newcommand{\curl}{\mathop{\mathrm{curl}}}
\def\Im{\mathop{\mathrm{Im}}}
\def\Re{\mathop{\mathrm{Re}}}
\newcommand{\Ei}{\mathop{\mathrm{Ei}}}
\newcommand{\Ci}{\mathop{\mathrm{Ci}}}
\newcommand{\Si}{\mathop{\mathrm{Si}}}
\newcommand{\sign}{\mathop{\mathrm{sign}}}
\newcommand{\Res}{\mathop{\mathrm{Res}}}
\newcommand{\arctanh}{\mathop{\mathrm{arctanh}}}

%Definitions: sets
\def\Lin{\ensuremath{\mathsf{Lin}}}
\def\Orth{\ensuremath{\mathsf{Orth}}}
\def\Sym{\ensuremath{\mathsf{Sym}}}
\newcommand{\Reals}{\ensuremath{\mathbb{R}}}
\newcommand{\Complex}{\ensuremath{\mathbb{C}}}
\newcommand{\Naturals}{\ensuremath{\mathbb{N}}}

%Definitions: journals
\def\AAM{{\it Arch.\ Appl.\ Mech.}\ }
\def\ACIJ{{\it ACI J.}\ }
\def\ACISJ{{\it ACI Struct.\ J.}\ }
\def\ACSB{{\it Am.\ Ceram.\ Soc.\ Bull.}\ }
\def\AM{{\it Acta mater.}\ }
\def\AMPA{{\it Ann.\ Mat.\ Pur.\ Appl.}\ }
\def\AMR{{\it Appl.\ Mech.\ Rev.}\ }
\def\ARMA{{\it Arch.\ Ration.\ Mech.\ An.}\ }
\def\CACS{{\it Comm.\ Am.\ Cer.\ Soc.}\ }
\def\CMAME{{\it Comput.\ Method.\ Appl.\ M.}\ }
\def\EFM{{\it Eng.\ Fract.\ Mech.}\ }
\def\EJMA{{\it Eur.\ J.\ Mech. A-Solid.}\ }
\def\IA{{\it Ing.\ Arch.}\ }
\def\IMA{{\it IMA J.\ Appl.\ Math.}\ }
\def\IJES{{\it Int.\ J.\ Eng.\ Sci.}\ }
\def\IJF{{\it Int.\ J.\ Fracture}\ }
\def\IJMS{{\it Int.\ J.\ Mech.\ Sci.}\ }
\def\IJNAMG{{\it Int.\ J.\ Numer.\ Anal.\ Meth.\ Geomech.}\ }
\def\IJNME{{\it Int.\ J.\ Numer.\ Meth.\ Eng.}\ }
\def\IJP{{\it Int.\ J.\ Plasticity}\ }
\def\IJSS{{\it Int.\ J.\ Solids Struct.}\ }
\def\JACS{{\it J.\ Am.\ Ceram.\ Soc.}\ }
\def\JAM{{\it ASME J.\ Appl.\ Mech.}\ }
\def\JAP{{\it J.\ Appl.\ Phys.}\ }
\def\JE{{\it J.\ Elasticity}\ }
\def\JEM{{\it ASCE J.\ Eng.\ Mech.}\ }
\def\JEMD{{\it ASCE J.\ Eng.\ Mech.\ Div.}\ }
\def\JEMT{{\it ASME J.\ Eng.\ Mater.\ Tech.}\ }
\def\JM{{\it J.\ M\'ecanique}\ }
\def\JMPS{{\it J.\ Mech.\ Phys.\ Solids}\ }
\def\JSHA{{\it J.\ Soc.\ Hungarian Arch.}\ }
\def\MCFM{{\it Mech.\ Cohes-Frict.\ Mat.}\ }
\def\MCM{{\it Mech.\ Compos.\ Mater.}\ }
\def\MDPM{{\it Mod.\ Dev.\ Powder Metall.}\ }
\def\ME{{\it Mater.\ Eng.}\ }
\def\MMS{{\it Math.\ Mech.\ Solids}\ }
\def\MOM{{\it Mech.\ Materials}\ }
\def\MPCPS{{\it Math.\ Proc.\ Camb.\ Phil.\ Soc.}\ }
\def\MRC{{\it Mech.\ Res.\ Commun.}\ }
\def\MRSB{{\it MRS Bull.}\ }
\def\MSE{{\it Mater.\ Sci.\ Eng.}\ }
\def\NED{{\it Nucl.\ Eng.\ Des.}\ }
\def\PM{{\it Phil.\ Mag.}\ }
\def\PRSL{{\it Proc.\ R.\ Soc.\ Lond.}\ }
\def\QAM{{\it Quart.\ Appl.\ Math.}\ }
\def\QJMAM{{\it Quart.\ J.\ Mech.\ Appl.\ Math.}\ }
\def\SF{{\it Soils Found.}\ }
\def\ZAMP{{\it Z.\ Angew.\ Math.\ Phys.}\ }
\def\ZAMM{{\it Z.\ Angew.\ Math.\ Mech.}\ }
\def\ZP{{\it Z.\ Phys.}\ }
